Logic-based Benders Decomposition and Binary Decision Diagram Based Approaches for Stochastic Distributed Operating Room Scheduling

The distributed operating room (OR) scheduling problem aims to find an assignment of surgeries to ORs across collaborating hospitals that share their waiting lists and ORs. We propose a stochastic extension of this problem where surgery durations are considered to be uncertain. In order to obtain solutions for the challenging stochastic model, we use sample average approximation, and develop two enhanced decomposition frameworks that use logic-based Benders (LBBD) optimality cuts and binary decision diagram based Benders cuts. Specifically, to the best of our knowledge, deriving LBBD optimality cuts in a stochastic programming context is new to the literature. Our computational experiments on a hospital dataset illustrate that the stochastic formulation generates robust schedules, and that our algorithms improve the computational efficiency.

==> Abstract.tex <==
The distributed operating room (OR) scheduling problem aims to find an assignment of surgeries to ORs across collaborating hospitals that share their waiting lists and ORs. We propose a stochastic extension of this problem where surgery durations are considered to be uncertain. In order to obtain the solutions for the stochastic model, we use sample average approximation, and develop two enhanced decomposition frameworks that use logic-based Benders (LBBD) optimality cuts and binary decision diagram based Benders cuts. Specifically, deriving LBBD optimality cuts in a stochastic programming context is new to the literature. Our computational experiments on a real-life hospital dataset illustrate that the stochastic formulation generates robust schedules, and that our algorithms improve the computational efficiency. 

==> AppendDors.tex <==
{\cred \section{Deterministic Distributed OR Scheduling (DORS) Problem}\label{chapter: dors}
For ease of comparison, we copy the deterministic DORS model from \cite{roshanaei2017propagating} in this section. The notations have the same meanings as what we use in the main paper, and are listed in Table \ref{table: SDORS_notation}.
\begin{subequations}\label{model: dors}
\begin{alignat}{5}
\text{(SDORS):} \ \min~~&\sum_{h\in\mc{H}} \sum_{d\in\mc{D}} G_{hd}u_{hd}+\sum_{h\in\mc{H}}\sum_{d\in\mc{D}}\sum_{r\in\mc{R}_h}F_{hd}y_{hdr}+\sum_{h\in\mc{H}}\sum_{d\in\mc{D}}\sum_{p\in\mc{P}}\sum_{r\in\mc{R}_h}c^{\text{sched}}_{dp}x_{hdpr}+  \hspace*{-5cm}\nonumber\\
&\sum_{p\in\mc{P} \setminus \mc{P'}}c^{\text{unsched}}_{p}w_p \hspace*{-5cm} &&\label{eq: dors_obj}\tag{A1}\\
\st ~~& \sum_{h\in\mc{H}}\sum_{d\in\mc{D}}\sum_{r\in\mc{R}_h}x_{hdpr}=1 & & \forall p \in \mc{P'} \label{eq: dors_assign_madatory_patients}\tag{A2}\\
      & \sum_{h\in\mc{H}}\sum_{d\in\mc{D}}\sum_{r\in\mc{R}_h}x_{hdpr}+w_p=1 & & \forall p \in \mc{P}\setminus\mc{P'} \label{eq: dors_assign_nonmandatory_patients}\tag{A3}\\
      &\sum_{p\in\mc{P}} T_p x_{hdpr} \leq B_{hd}y_{hdr} && \forall h\in\mc{H}, d\in\mc{D}, r\in\mc{R}_h  \label{eq: dors_time_limit}\tag{A4} \\
      & y_{hdr}\leq y_{hd,r-1} & &\forall h\in \mc{H}, d\in\mc{D},r\in\mc{R}_h\setminus\{1\} \label{eq: dors_symmetry_breaking_y}\tag{A5} \\
     & y_{hdr}\leq u_{hd}& &\forall h\in \mc{H}, d\in\mc{D}, r\in\mc{R}_h \label{eq: dors_y-u}\tag{A6} \\
     & x_{hdpr}\leq y_{hdr} & &\forall h\in \mc{H}, d\in\mc{D}, p\in \mc{P}, r\in\mc{R}_h \label{eq: dors_x-y}\tag{A7} \\
%     & \sum_{p\in\mc{P}} T^s_p (x_{hdpr}-z^s_{hdpr}) \leq B_{hd}y_{hdr} && \forall h\in\mc{H}, d\in\mc{D}, r\in\mc{R}_h, s\in\mc{S} \label{eq: dors_time_limit} \\
%     & z^s_{hdpr}\leq x_{hdpr}  & & \forall h\in\mc{H}, d\in\mc{D}, p\in\mc{P}, r\in\mc{R}_h,  s\in\mc{S} \label{eq: dors_z-x} \\
     & u_{hd},y_{hdr},x_{hdpr}, w_p\in \{0,1\} & &\forall h\in \mc{H}, d\in\mc{D}, p\in \mc{P}, r\in\mc{R}_h\label{eq: dors_binary}\tag{A8}
\end{alignat}
\end{subequations}

The objective function \eqref{eq: dors_obj} minimizes the total operational cost. Constraints \eqref{eq: dors_assign_madatory_patients} ensure that mandatory patients are all scheduled in the current planning horizon. Constraints \eqref{eq: dors_assign_nonmandatory_patients} either schedule non-mandatory patients in the current planning horizon or postpone their surgeries to a future time. Constraints \eqref{eq: dors_time_limit} ensure that the surgeries scheduled in an OR will not exceed the OR's operating time limit.  Constraints \eqref{eq: dors_symmetry_breaking_y} are symmetry breaking constraints for ORs in the same hospital, since they are homogeneous. Constraints \eqref{eq: dors_y-u} link $u$ and $y$ variables, to ensure that if the surgical suite in a hospital is closed, no OR in it is opened. Similarly, constraints \eqref{eq: dors_x-y} make sure that a patient will only be assigned to an opened OR. Lastly, constraints \eqref{eq: dors_binary} enforce binary restrictions on the decision variables.

Note that compared with \cite{roshanaei2017propagating}, the last two terms of the objective are simplified, substituting the expressions for costs $\kappa_1\rho_p(d-\alpha_p)$ and $\kappa_2\rho_p(|\mc{D}| + 1 -\alpha_p)$ with equivalent notations $c^{\text{sched}}_{dp}$ and $c^{\text{unsched}}_p$.
}

==> AppendExample.tex <==
\section{Simple Example for BDD}\label{chapter: app_example}
The following simple example provides an illustration of the BDD transformation. Suppose in {\cred the subproblem \eqref{model: sors_sub}} for an $(h, d, r, s)$ tuple there are four scheduled patients, and we need to decide whether to cancel them. The subproblem formulation is the following {\cred (we have replaced all $\hat{x}_{hdp}, p =1,...,4$ in subproblem \eqref{model: sors_sub} with 1, as all four patients are selected)}:
\begin{align*}
{\cred \bar{Q}_{hdr}^s = \min} \ & 4(1 - z^s_{hd1r})+(1- z^s_{hd2r})+3(1- z^s_{hd3r})+8(1-z^s_{hd4r}) &&\\
\text{s.t.} \ & {\cred 2z^s_{hd1r}+z^s_{hd2r}+3z^s_{hd3r}+3z^s_{hd4r} \leq 5}&& \\
&z^s_{hdpr}  \leq 1 &&\forall p\in\hat{\mc{P}}_{hdr}\\
& z^s_{hdpr} \in \{0,1\} &&\forall p\in\hat{\mc{P}}_{hdr}
\end{align*}
where $\hat{\mc{P}}_{hdr} = \{1,2,3,4\}$ {\cred represents the subset of selected patients. To simplify the notation, we equivalently rewrite the objective as:} 
\begin{align*}
{\cred \bar{Q}_{hdr}^s - 16 = \min~~ - 4z^s_{hd1r} - z^s_{hd2r} - 3z^s_{hd3r} - 8z^s_{hd4r}}
\end{align*}

The problem is reformulated via the BDD in Figure \ref{fig: bdd_example}. The BDD contains a root node at the top, denoted by $o$, and a terminal node at the bottom, denoted by $t$. Each layer of the arcs represents the values of the variables $z^s_{hdpr}$, from patient 1 to patient 4. Notice that the patients can be sorted in a different way from the order in the graph, and that will produce a different BDD, thus may result in different computational performance. At each layer, the dashed and solid arcs respectively indicate selecting 0 and 1 values for the layer's corresponding variable. The value above or beside each arc is the cost of $z^s_{hdpr}$ if it receives the value indicated by the arc type. When transferring the subproblem to a shortest path problem, those values are used as costs for the arcs. Each route from the node $o$ to the node $t$ represents a feasible solution for the subproblem, and each feasible solution is represented by a route from the node $o$ to the node $t$. Also, the path length provides the correct evaluation of the objective value for a corresponding feasible solution. Therefore, by finding a shortest path from the root node to the terminal node, we are able to obtain an optimal solution to the subproblem. 

\input{bdd_figure}
%\newpage
